A Comprehensive Survey on Deep Clustering: Taxonomy, Challenges, and Future Directions

Clustering is a fundamental machine learning task which has been widely studied in the literature. Classic clustering methods follow the assumption that data are represented as features in a vectorized form through various representation learning techniques. As the data become increasingly complicated and complex, the shallow (traditional) clustering methods can no longer handle the high-dimensional data type. With the huge success of deep learning, especially the deep unsupervised learning, many representation learning techniques with deep architectures have been proposed in the past decade. Recently, the concept of Deep Clustering, i.e., jointly optimizing the representation learning and clustering, has been proposed and hence attracted growing attention in the community. Motivated by the tremendous success of deep learning in clustering, one of the most fundamental machine learning tasks, and the large number of recent advances in this direction, in this paper we conduct a comprehensive survey on deep clustering by proposing a new taxonomy of different state-of-the-art approaches. We summarize the essential components of deep clustering and categorize existing methods by the ways they design interactions between deep representation learning and clustering. Moreover, this survey also provides the popular benchmark datasets, evaluation metrics and open-source implementations to clearly illustrate various experimental settings. Last but not least, we discuss the practical applications of deep clustering and suggest challenging topics deserving further investigations as future directions.

==> comparetable.tex <==
\begin{table*}[!htbp]
    \centering
    \begin{tabularx}{\textwidth}{|X|X|X|X|X|X|}
 \hline
        \multirow{2}{*}{taxonomy}        
        & \multicolumn{2}{c|}{Advantages}      
        & \multicolumn{2}{c|}{Disadvantages}   
\\  \cline{2-5}
               
        &adv1    
        &adv2
        &Error Propagation
        &div2
        
\\ \hline
        Multi Stage
        &$ \checkmark $    
        &
        &
        &                 
\\ \hline
        
        Generative 
        &    
        &$ \checkmark $  
        &
        &                          
\\ \hline
        
        Iterative       
        &    
        &
        &$ \checkmark $  
        &                          
\\ \hline

        Simultaneously  
        &    
        &
        &
        &$ \checkmark $                            
\\ \hline
    \end{tabularx}%
    \label{table:comparisons}
    \caption{ Advantages and disadvantages analysis}
\end{table*}%

==> list.tex <==
% \subsection{Deep Generative Clustering}
% \begin{enumerate}
%     \item $\color{green}\checkmark$ (IJCAI2017) Variational Deep Embedding: An Unsupervised and Generative Approach to Clustering\cite{jiang2016variational}
%     \item $\color{green}\checkmark$ (CVPR2018) Balanced Self-Paced Learning for Generative Adversarial Clustering Network\cite{ghasedi2019balanced}
%     \item $\color{green}\checkmark$ (IJCNN2020) Variational Clustering: Leveraging Variational Autoencoders for Image Clustering\cite{prasad2020variational}
%     \item $\color{green}\checkmark$ (IJCNN2020) Unsupervised Clustering through Gaussian Mixture Variational AutoEncoder with Non-Reparameterized Variational Inference and Std Annealing\cite{li2020unsupervised}
%     \item $\color{green}\checkmark$ (Arxiv2016) Deep unsupervised clustering with gaussian mixture variational autoencoders\cite{dilokthanakul2016deep}
%     \item $\color{green}\checkmark$ (AAAI2019) Clustergan: Latent space clustering in generative adversarial networks\cite{mukherjee2019clustergan}
%     \item $\color{green}\checkmark$ (ICCV2019) Deep clustering by gaussian mixture variational autoencoders with graph embedding\cite{yang2019deep}
%     \item $\color{green}\checkmark$ (TNNLS2021) Image clustering using an augmented generative adversarial network and information maximization\cite{ntelemis2021image}
%     \item $\color{green}\checkmark$ (TNNLS2021)A Decoder-Free Variational Deep Embedding for Unsupervised Clustering\cite{ji2021decoder}
%     \item $\color{green}\checkmark$ Neural Mixture Models with Expectation-Maximization for End-to-end Deep Clustering
%     \item $\color{green}\checkmark$ Deep Distribution-preserving Incomplete Clustering with Optimal Transport
%     \item Neural generative model for clustering by separating particularity and commonality
%     \item $\color{green}\checkmark$ (Arxiv2018) Gaussian mixture generative adversarial networks for diverse datasets, and the unsupervised clustering of images
%     \item (ECCV2020) Deep Image Clustering with Category-Style Representation\cite{zhao2020deep}
%     \item $\color{green}\checkmark$ (IJCAI'18) Mixture of GANs for Clustering \cite{yu2018mixture}
%     \item Learning the Precise Feature for Cluster Assignment
% \end{enumerate}



% \subsection{Iterative Deep Clustering}
% \begin{enumerate}
%     \item $\color{green}\checkmark$(CVPR2016) Joint unsupervised learning of deep representations and image clusters\cite{yang2016joint}
%     \item $\color{green}\checkmark$(ICML2017) Towards K-means-friendly Spaces: Simultaneous Deep Learning and Clustering\cite{yang2017towards}
%     \item $\color{green}\checkmark$(ECCV2020) GATCluster: Self-supervised Gaussian-Attention Network for Image Clustering \cite{niu2020gatcluster}
% \end{enumerate}

% \subsubsection{Pseudo Labeling}
% \begin{enumerate}
%     % \item (ECCV2020) Scan: Learning to classify images without labels\cite{van2020scan}
%     % \item (ICCV2017) Deep Adaptive Image Clustering\cite{chang2017deep}
%     % \item (ECMLPKDD2017) Deepcluster: A general clustering framework based on deep learning\cite{tian2017deepcluster}
%     % \item (Arxiv2021) Spice: Semantic pseudo-labeling for image clustering\cite{niu2021spice}
%     %   \item (ICLR 2020) Self-labelling via simultaneous clustering and representation learning\cite{asano2019self}
% \end{enumerate}

% \subsubsection{Subspace Clustering(Pseudo labeling)}
% \begin{enumerate}
%     \item $\color{green}\checkmark$(CVPR2019) Self-supervised convolutional subspace clustering network\cite{zhang2019self}
%     \item $\color{green}\checkmark$(TIP2021) Pseudo-supervised deep subspace clustering\cite{lv2021pseudo}
%     \item $\color{green}\checkmark$(ICML2019) Neural collaborative subspace clustering\cite{zhang2019neural}
% \end{enumerate}

% \subsubsection{Auto-encoder based Deep Clustering}
% \begin{enumerate}
%     \item $\color{green}\checkmark$(CIARP2013) Auto-encoder Based Data Clustering\cite{song2013auto}
%     \item $\color{green}\checkmark$(TKDE2020) Adversarial Deep Embedding Clustering On a better Trade-off between Feature Randomness and Feature Drift\cite{mrabah2020adversarial}
% \end{enumerate}




% \subsection{Simultaneously Deep Clustering}
% \begin{enumerate}
%     \item (DEC's $L_{st}$+Subspace clustering)$\color{green}\checkmark$(AAAI2017)Cascade subspace clustering\cite{peng2017cascade}
% \end{enumerate}

% \subsubsection{Clustering with constrarints}
% \begin{enumerate}
%         \item $\color{red}\checkmark$ $\color{green}\checkmark$(CVPR2019)(DDC) Deep Discriminative clustering analysis\cite{chang2019deep}
% \end{enumerate}


% \subsubsection{Contrastive Learning based Deep Clustering}
% \begin{enumerate}
    % \item $\color{red}\checkmark$ $\color{green}\checkmark$(ICCV2019)(DCCM) Deep Comprehensive Correlation Mining for Image Clustering\cite{wu2019deep}
    % \item $\color{red}\checkmark$ $\color{green}\checkmark$(ECCV2020) (DCCS)Deep Image Clustering with Category-Style Representation\cite{zhao2020deep}
    % \item $\color{green}\checkmark$(CVPR2020)(PICA) Deep Semantic Clustering by Partition Confidence Maximisation\cite{huang2020deep}
    % \item $\color{green}\checkmark$(ICCV2019)(IIC) Invariant information clustering for unsupervised image classification and segmentation\cite{ji2019invariant}
    % \item $\color{green}\checkmark$(Arxiv2020)(DRC) Deep Robust Clustering by Contrastive Learning\cite{zhong2020deep}
    % \item $\color{green}\checkmark$(ICLR2020) Mice: Mixture of contrastive experts for unsupervised image clustering\cite{tsai2020mice}
    % \item $\color{green}\checkmark$(ICPR2020) Multi-Modal Deep Clustering: Unsupervised Partitioning of Images\cite{shiran2021multi}
    % \item $\color{green}\checkmark$(Arxiv2020) Deep robust clustering by contrastive learning\cite{zhong2020deep}
    % \item $\color{green}\checkmark$(ICCV2021) Graph Contrastive Clustering \cite{zhong2021graph}
    % \item $\color{green}\checkmark$(IJCAI2021) Deep Descriptive Clustering\cite{zhang2021deep}
    % \item $\color{red}\checkmark$ $\color{green}\checkmark$(AAAI2021) Contrastive Clustering\cite{li2021contrastive}
    % \item (TNNLS2021) A Decoder-Free Variational Deep Embedding for Unsupervised Clustering\cite{ji2021decoder}
    % \item $\color{green}\checkmark$(Arxiv2021) Doubly contrastive deep clustering\cite{dang2021doubly}
    % \item $\color{green}\checkmark$(Arxiv2021)(SCL) Deep clustering by semantic contrastive learning\cite{huang2021deep}
    % \item $\color{green}\checkmark$(NIPS2021) You Never Cluster Alone\cite{shen2021you}
    % \item $\color{green}\checkmark$(ICCV2021)(CRLC)Clustering by maximizing mutual information across views\cite{do2021clustering}
    % \item (ICPR2021) Variational Deep Embedding Clustering by Augmented Mutual Information Maximization\cite{ji2021variational}
    % \item $\color{green}\checkmark$(Arxiv2021)Information Maximization Clustering via Multi-View Self-Labelling\cite{ntelemis2021information}
    % \item $\color{green}\checkmark$(Arxiv2021) Exploring Non-Contrastive Representation Learning for Deep Clustering\cite{huang2021exploring}
    % \item $\color{green}\checkmark$(Arxiv2021) Cluster Analysis with Deep Embeddings and Contrastive Learning\cite{sundareswaran2021cluster}
    % \item $\color{green}\checkmark$(NAACL2021)(SCCL) Supporting clustering with contrastive learning\cite{zhang2021supporting}
% \end{enumerate}

% \subsubsection{Auto-encoder based Deep Clustering}
% \begin{enumerate}
%     \item $\color{green}\checkmark$(ICML2016) Unsupervised deep embedding for clustering analysis\cite{xie2016unsupervised} 
%     \item $\color{green}\checkmark$(IJCAI2017) Improved Deep Embedded Clustering with Local Structure Preservation\cite{guo2017improved}
%     \item $\color{green}\checkmark$(ICCV2017) Deep Clustering via Joint Convolutional Autoencoder Embedding and Relative Entropy Minimization\cite{ghasedi2017deep}
%     \item $\color{green}\checkmark$(CVPR2019) Deep Spectral Clustering using Dual Autoencoder Network\cite{yang2019deep}
%     \item $\color{green}\checkmark$(PR2018) Discriminatively Boosted Image Clustering with Fully Convolutional Auto-Encoders\cite{li2018discriminatively}
%     \item $\color{green}\checkmark$(PMLR2018) Deep Embedded Clustering with Data Augmentation\cite{guo2018deep}
%     \item $\color{green}\checkmark$(ICONIP2017) Deep Clustering with Convolutional Autoencoders\cite{guo2017deep}
%     \item $\color{green}\checkmark$(Arxiv2021)Learning Statistical Representation with Joint Deep Embedded Clustering\cite{rezaei2021learning}
% \end{enumerate}



\subsection{Not grouped yet}

% \subsubsection{simple combination}
% \begin{enumerate}
%     \item $\color{green}\checkmark$(PRL2020) Deep k-Means: Jointly clustering with k-Means and learning representations\cite{fard2020deep}
% \end{enumerate}

\subsubsection{Multi-stage}
\begin{enumerate}
    % \item $\color{green}\checkmark$(AAAI2014) Learning Deep Representations for Graph Clustering\cite{tian2014learning}
    % \item $\color{green}\checkmark$(ICPR2014) Deep Embedding Network for Clustering\cite{huang2014deep}
    \item (KBS2022) Deep image clustering by fusing contrastive learning and neighbor relation mining\cite{xu2022deep}
\end{enumerate}

% \subsubsection{Subspace Clustering(Multi-stage)}
% \begin{enumerate}
%     \item $\color{green}\checkmark$(NIPS2017) Deep Subspace Clustering Networks\cite{ji2017deep}
%     \item $\color{green}\checkmark$(CVPR2021) Learning a Self-Expressive Network for Subspace Clustering\cite{zhang2021learning}
%     \item $\color{green}\checkmark$(IJCAI 2016) Deep Subspace clustering with sparsity prior \cite{peng2016deep}
%     \item $\color{green}\checkmark$(CVPR2018) Deep Adversarial Subspace Clustering\cite{zhou2018deep}
% \end{enumerate}


\subsubsection{Multi-view Clustering}
\begin{enumerate}
    \item (CVPR2021) COMPLETER: Incomplete Multi-view Clustering via Contrastive Prediction\cite{lin2021completer}
    \item (TPAMI2021) Efficient and effective regularized incomplete multi-view clustering\cite{liu2020efficient}
    \item (ICCV2021) One-pass Multi-view Clustering for Large-scale Data\cite{liu2021one}  
    \item (AAAI2020) Unified graph and low-rank tensor learning for multi-view clustering\cite{wu2020unified}
\end{enumerate}

% \subsubsection{Subspace Clustering}
% \begin{enumerate}
%     \item $\color{green}\checkmark$(CVPR 2009)Sparse subspace clustering\cite{vidal2009sparse}
% \end{enumerate}

\subsubsection{Others}
\begin{enumerate}
    \item The single-noun prior for image clustering
    \item Agglomerative clustering using the concept of mutual nearest neighbourhood.
    \item Self-tuning spectral clustering
    \item Progressive self-supervised clustering with novel category discovery
    \item Associative deep clustering: Training a classiﬁcation network with no labels
    \item $\color{green}\checkmark$ (ICASS)Deep clustering: Discriminative embeddings for segmentation and separation%Deep Clustering开山鼻祖？
\end{enumerate}


\subsection{Representation Learning}
\begin{enumerate}
    \item $\color{green}\checkmark$ (CVPR 2018) Unsupervised Feature Learning via Non-Parametric Instance Discrimination\cite{wu2018unsupervised}
    % \item $\color{green}\checkmark$ Clustering-friendly representation learning via instance discrimination and feature decorrelation\cite{tao2021clustering}
    \item $\color{green}\checkmark$ (Arxiv 2021) Learning Representations by Contrasting Clusters While Bootstrapping Instances\cite{lee2020learning}
    % \item $\color{green}\checkmark$ (ICML 2017)Towards K-means-friendly spaces: Simultaneous deep learning and clustering\cite{yang2017towards}
    \item $\color{green}\checkmark$ Consensus Clustering With Unsupervised Representation Learning\cite{regatti2021consensus}
\end{enumerate}


\subsection{Application}
\begin{enumerate}
    \item $\color{green}\checkmark$(ICCV2021) End-to-end robust joint unsupervised image alignment and clustering\cite{zeng2021end}
\end{enumerate}





==> taxonomy.tex <==
In this section, we will summarize existing deep clustering methods based on the interaction between the representation learning module and clustering module.
More specifically, we summarize the following four deep clustering frameworks:
\begin{enumerate}
    \item Generative deep clustering: the clustering module is modeled as a prior of representation module.
    \item Iterative deep clustering: the representation learning module and the clustering module are iteratively updated.
    \item Simultaneous deep clustering: the representation learning module and the clustering module are simultaneously updated.
    \item Multi-stage deep clustering: the representation learning module is sequential connected with the clustering module.\
\end{enumerate}
Next, we will introduce the representative setting of each type of methods.

